PgNN: Physics-guided Neural Network for Fourier Ptychographic Microscopy

Fourier ptychography (FP) is a newly developed computational imaging approach that achieves both high resolution and wide field of view by stitching a series of low-resolution images captured under angle-varied illumination. So far, many supervised data-driven models have been applied to solve inverse imaging problems. These models need massive amounts of data to train, and are limited by the dataset characteristics. In FP problems, generic datasets are always scarce, and the optical aberration varies greatly under different acquisition conditions. To address these dilemmas, we model the forward physical imaging process as an interpretable physics-guided neural network (PgNN), where the reconstructed image in the complex domain is considered as the learnable parameters of the neural network. Since the optimal parameters of the PgNN can be derived by minimizing the difference between the model-generated images and real captured angle-varied images corresponding to the same scene, the proposed PgNN can get rid of the problem of massive training data as in traditional supervised methods. Applying the alternate updating mechanism and the total variation regularization, PgNN can flexibly reconstruct images with improved performance. In addition, the Zernike mode is incorporated to compensate for optical aberrations to enhance the robustness of FP reconstructions. As a demonstration, we show our method can reconstruct images with smooth performance and detailed information in both simulated and experimental datasets. In particular, when validated in an extension of a high-defocus, high-exposure tissue section dataset, PgNN outperforms traditional FP methods with fewer artifacts and distinguishable structures.

==> 8.reference.tex <==
% Can use something like this to put references on a page
% by themselves when using endfloat and the captionsoff option.

\ifCLASSOPTIONcaptionsoff
  \newpage
\fi


% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

%% references section
\begin{thebibliography}{40}

\bibitem{1}% 1
G. Zheng, R. Horstmeyer, and C. Yang, “Wide-field, high-resolution Fourier ptychographic microscopy,” Nat Photonics, vol. 7, no. 9, pp. 739-745, Sep 1, 2013.

\bibitem{2}% 2
X. Ou, G. Zheng, and C. Yang, “Embedded pupil function recovery for Fourier ptychographic microscopy,” Opt Express, vol. 22, no. 5, pp. 4960-72, Mar 10, 2014.

\bibitem{3}% 3
L. Tian, X. Li, K. Ramchandran, and L. Waller, “Multiplexed coded illumination for Fourier Ptychography with an LED array microscope,” Biomedical optics express, vol. 5, no. 7, pp. 2376-2389, 2014.

\bibitem{4}% 4
J. R. Fienup, “Reconstruction of a complex-valued object from the modulus of its Fourier transform using a support constraint,” JOSA A, vol. 4, no. 1, pp. 118-123, 1987.

\bibitem{5}% 5
J. R. Fienup, “Phase retrieval algorithms: a personal tour,” Applied optics, vol. 52, no. 1, pp. 45-56, 2013.

\bibitem{6}% 6
V. Mico, Z. Zalevsky, P. García-Martínez, and J. García, “Synthetic aperture superresolution with multiple off-axis holograms,” JOSA A, vol. 23, no. 12, pp. 3162-3170, 2006.

\bibitem{7}% 7
L. Granero, V. Micó, Z. Zalevsky, and J. García, “Synthetic aperture superresolved microscopy in digital lensless Fourier holography by time and angular multiplexing of the object information,” Applied optics, vol. 49, no. 5, pp. 845-857, 2010.

\bibitem{8}% 8
A. Sinha, J. Lee, S. Li, and G. Barbastathis, “Lensless computational imaging through deep learning,” Optica, vol. 4, no. 9, pp. 1117-1125, 2017.

\bibitem{9}% 9
A. M. Maiden, and J. M. Rodenburg, “An improved ptychographical phase retrieval algorithm for diffractive imaging,” Ultramicroscopy, vol. 109, no. 10, pp. 1256-62, Sep, 2009.

\bibitem{10}% 10
J. Chung, X. Ou, R. P. Kulkarni, and C. Yang, “Counting White Blood Cells from a Blood Smear Using Fourier Ptychographic Microscopy,” PLoS One, vol. 10, no. 7, pp. e0133489, 2015.

\bibitem{11}% 11
R. Horstmeyer, X. Ou, G. Zheng, P. Willems, and C. Yang, “Digital pathology with Fourier ptychography,” Comput Med Imaging Graph, vol. 42, pp. 38-43, Jun, 2015.

\bibitem{12}% 12
K. Guo, S. Dong, P. Nanda, and G. Zheng, “Optimization of sampling pattern and the design of Fourier ptychographic illuminator,” Opt Express, vol. 23, no. 5, pp. 6171-80, Mar 9, 2015.

\bibitem{13}% 13
K. Guo, Z. Bian, S. Dong, P. Nanda, Y. M. Wang, and G. Zheng, “Microscopy illumination engineering using a low-cost liquid crystal display,” Biomed Opt Express, vol. 6, no. 2, pp. 574-9, Feb 1, 2015.

\bibitem{14}% 14
A. Kappeler, S. Ghosh, J. Holloway, O. Cossairt, and A. Katsaggelos, "PtychNet: CNN based Fourier ptychography." pp. 1712-1716.

\bibitem{15}% 15
T. Nguyen, Y. Xue, Y. Li, L. Tian, and G. Nehmetallah, “Convolutional neural network for Fourier ptychography video reconstruction: learning temporal dynamics from spatial ensembles,” arXiv preprint arXiv:1805.00334, 2018.

\bibitem{16}% 16
Y. Rivenson, Y. Zhang, H. Gunaydin, D. Teng, and A. Ozcan, “Phase recovery and holographic image reconstruction using deep learning in neural networks,” Light Sci Appl, vol. 7, pp. 17141, 2018.

\bibitem{17}% 17
J. Zhang, T. Xu, Z. Shen, Y. Qiao, and Y. Zhang, “Fourier ptychographic microscopy reconstruction with multiscale deep residual network,” Opt Express, vol. 27, no. 6, pp. 8612-8625, Mar 18, 2019.

\bibitem{18}% 18
M. Kellman, E. Bostan, M. Chen, and L. Waller, “Data-Driven Design for Fourier Ptychographic Microscopy,” arXiv preprint arXiv:1904.04175, 2019.

\bibitem{19}% 19
Y. F. Cheng, M. Strachan, Z. Weiss, M. Deb, D. Carone, and V. Ganapati, “Illumination pattern design with deep learning for single-shot Fourier ptychographic microscopy,” Opt Express, vol. 27, no. 2, pp. 644-656, Jan 21, 2019.

\bibitem{20}% 20
M. Kellman, E. Bostan, N. Repina, and L. Waller, “Physics-based Learned Design: Optimized Coded-Illumination for Quantitative Phase Imaging,” IEEE Transactions on Computational Imaging, 2019.

\bibitem{21}% 21
S. Jiang, K. Guo, J. Liao, and G. Zheng, “Solving Fourier ptychographic imaging problems via neural network modeling and TensorFlow,” Biomedical optics express, vol. 9, no. 7, pp. 3306-3319, 2018.

\bibitem{22}% 22
A. Lucas, M. Iliadis, R. Molina, and A. K. Katsaggelos, “Using Deep Neural Networks for Inverse Problems in Imaging: Beyond Analytical Methods,” IEEE Signal Processing Magazine, vol. 35, no. 1, pp. 20-36, 2018.

\bibitem{23}% 23
J. Kyong Hwan, M. T. McCann, E. Froustey, and M. Unser, “Deep Convolutional Neural Network for Inverse Problems in Imaging,” IEEE Trans Image Process, vol. 26, no. 9, pp. 4509-4522, Sep, 2017.

\bibitem{24}% 24
C. Dong, C. C. Loy, K. He, and X. Tang, “Image Super-Resolution Using Deep Convolutional Networks,” IEEE Trans Pattern Anal Mach Intell, vol. 38, no. 2, pp. 295-307, Feb, 2016.

\bibitem{25}% 25
S. Wang, Z. Su, L. Ying, X. Peng, S. Zhu, F. Liang, D. Feng, and D. Liang, "Accelerating magnetic resonance imaging via deep learning." pp. 514-517.

\bibitem{26}% 26
G. Yang, S. Yu, H. Dong, G. Slabaugh, P. L. Dragotti, X. Ye, F. Liu, S. Arridge, J. Keegan, Y. Guo, D. Firmin, J. Keegan, G. Slabaugh, S. Arridge, X. Ye, Y. Guo, S. Yu, F. Liu, D. Firmin, P. L. Dragotti, G. Yang, and H. Dong, “DAGAN: Deep De-Aliasing Generative Adversarial Networks for Fast Compressed Sensing MRI Reconstruction,” IEEE Trans Med Imaging, vol. 37, no. 6, pp. 1310-1321, Jun, 2018.

\bibitem{27}% 27
Z. Ren, Z. Xu, and E. Y. Lam, “Learning-based nonparametric autofocusing for digital holography,” Optica, vol. 5, no. 4, pp. 337, 2018.

\bibitem{28}% 28
Y. Wu, Y. Rivenson, Y. Zhang, Z. Wei, H. Günaydin, X. Lin, and A. Ozcan, “Extended depth-of-field in holographic imaging using deep-learning-based autofocusing and phase recovery,” Optica, vol. 5, no. 6, pp. 704, 2018.

\bibitem{29}% 29
P. Klages, I. Bensilmane, S. Ryahi, J. Jiang, M. Hunt, J. Deasy, and N. Tyagi, “Comparison of Patch-Based Conditional Generative Adversarial Neural Net Models with Emphasis on Model Robustness for Use in Head and Neck Cases for MR-Only planning,” arXiv preprint arXiv:1902.00536, 2019.

\bibitem{30}% 30
J. Jiang, Y. C. Hu, N. Tyagi, P. Zhang, A. Rimner, G. S. Mageras, J. O. Deasy, and H. Veeraraghavan, “Tumor-aware, Adversarial Domain Adaptation from CT to MRI for Lung Cancer Segmentation,” Med Image Comput Comput Assist Interv, vol. 11071, pp. 777-785, Sep, 2018.

\bibitem{31}% 31
C. Metzler, A. Mousavi, and R. Baraniuk, "Learned D-AMP: Principled neural network based compressive image recovery." pp. 1772-1783.

\bibitem{32}% 32
H. He, C.-K. Wen, S. Jin, and G. Y. Li, “Deep Learning-Based Channel Estimation for Beamspace mmWave Massive MIMO Systems,” IEEE Wireless Communications Letters, vol. 7, no. 5, pp. 852-855, 2018.

\bibitem{33}% 33
J. Liao, Y. Jiang, Z. Bian, B. Mahrou, A. Nambiar, A. W. Magsam, K. Guo, S. Wang, Y. K. Cho, and G. Zheng, “Rapid focus map surveying for whole slide imaging with continuous sample motion,” Opt Lett, vol. 42, no. 17, pp. 3379-3382, Sep 1, 2017.

\bibitem{34}% 34
L. H. Yeh, J. Dong, J. Zhong, L. Tian, M. Chen, G. Tang, M. Soltanolkotabi, and L. Waller, “Experimental robustness of Fourier ptychography phase retrieval algorithms,” Opt Express, vol. 23, no. 26, pp. 33214-40, Dec 28, 2015.

\bibitem{35}% 35
Y. Yang, Z. Zhong, T. Shen, and Z. Lin, "Convolutional neural networks with alternately updated clique." pp. 2413-2422.

\bibitem{36} %36
A. Kappeler, S. Yoo, Q. Dai, and A. K. Katsaggelos, “Video Super-Resolution With Convolutional Neural Networks,” IEEE Transactions on Computational Imaging, vol. 2, no. 2, pp. 109-122, 2016.

\bibitem{37} %37
A. Mahendran, and A. Vedaldi, "Understanding deep image representations by inverting them." pp. 5188-5196.

\bibitem{38} %38
L. N. Thibos, R. A. Applegate, J. T. Schwiegerling, and R. Webb, “Standards for reporting the optical aberrations of eyes,” Journal of refractive surgery, vol. 18, no. 5, pp. S652-S660, 2002.

\end{thebibliography}

